Comparing the pre-SNe feedback and environmental pressures for 6000 HII regions across 19 nearby spiral galaxies

The feedback from young stars (i.e. pre-supernova) is thought to play a crucial role in molecular cloud destruction. In this paper, we assess the feedback mechanisms acting within a sample of 5810 HII regions identified from the PHANGS-MUSE survey of 19 nearby ($<$ 20 Mpc) star-forming, main sequence spiral galaxies (log($M_\star$/M$_\odot$)= 9.4 $-$ 11). These optical spectroscopic maps are essential to constrain the physical properties of the HII regions, which we use to investigate their internal pressure terms. We estimate the photoionised gas ($P_\mathrm{therm}$), direct radiation ($P_\mathrm{rad}$), and mechanical wind pressure ($P_\mathrm{wind}$), which we compare to the confining pressure of their host environment ($P_\mathrm{de}$). The HII regions remain unresolved within our ${\sim}50{-}100$ pc resolution observations, so we place upper ($P_\mathrm{max}$) and lower ($P_\mathrm{min}$) limits on each of the pressures by using a minimum (i.e. clumpy structure) and maximum (i.e. smooth structure) size, respectively. We find that the $P_\mathrm{max}$ measurements are broadly similar, and for $P_\mathrm{min}$ the $P_\mathrm{therm}$ is mildly dominant. We find that the majority of HII regions are over-pressured, $P_\mathrm{tot}/P_\mathrm{de} = (P_\mathrm{therm}+P_\mathrm{wind}+P_\mathrm{rad})/P_\mathrm{de} > 1$, and expanding, yet there is a small sample of compact HII regions with $P_\mathrm{tot,max}/P_\mathrm{de} < 1$ ($\sim$1% of the sample). These mostly reside in galaxy centres ($R_\mathrm{gal}<1$kpc), or, specifically, environments of high gas surface density; log($\Sigma_\mathrm{gas}/\mathrm{M_\odot} \mathrm{pc}^{-2}$)$\sim$2.5 (measured on kpc-scales). Lastly, we compare to a sample of literature measurements for $P_\mathrm{therm}$ and $P_\mathrm{rad}$ to investigate how dominant pressure term transitions over around 5dex in spatial dynamic range and 10 dex in pressure.

==> figs/fig_Rfrac.tex <==
\begin{figure}
    \centering
	\includegraphics[width=0.95\columnwidth]{figs/scatter/rad_halum_anno_compressed.pdf}
    \caption{The extinction corrected luminosity of \Ha\ as a function of the effective radius for the \HII\ region sample. Shown as a diagonal dashed black line is a power-law fit to all the data points. The horizontal dotted line shows the $3\,\times\,10^{36}$\,\ergs\ luminosity threshold, which, based on the fitted power-law relation, we expect sources below this to be mostly unresolved throughout our sample. We use the distribution of sources below this luminosity threshold to define a relative size threshold of $r_\mathrm{eff}/r_\mathrm{eff, min}=2$ where $r_\mathrm{eff, min}$ is the minimum effective radius measured within each galaxy. We highlight above (resolved) and below (unresolved) as orange and green points, respectively.}
    \label{fig:plot_Rlum}
\end{figure}


\begin{figure}
    \centering
	\includegraphics[width=1\columnwidth]{figs/hist/hist_radiusfracanno_compressed.pdf}
    \caption{Histogram of the relative size distribution for the \HII\ region sample. Shown is the ratio of the effective radius of each \HII\ region ($r_\mathrm{eff}$) and the minimum \HII\ region radius measured within its host galaxy ($r_\mathrm{eff,min}$). We plot the complete sample of \HII\ regions in orange. We plot the faint \HII\ regions we expect to be unresolved in blue; i.e. those with an extinction-corrected \Ha\ luminosity $<\,3\,\times\,10^{36}$\,\ergs, and given the \HII\ region size-luminosity relation and our surface brightness limit. We use this to define the requirement that $r_\mathrm{eff}/r_\mathrm{eff,min}>2$ for a \HII\ region within the sample to be resolved.}
    \label{fig:hist_Rfrac}
\end{figure}


==> figs/fig_presscaterr.tex <==
\begin{figure*}
    \centering
	\includegraphics[width=0.9\textwidth]{figs/scatter/rad_pallerr_anno_compressed.pdf}
    \caption{{\em Left:} Thermal and direct radiation pressure components as a function of effective radius. We highlight the approximate collection of points that are consider to be unresolved ($r_\mathrm{eff}/r_\mathrm{eff,min}$<2) and resolved ($r_\mathrm{eff}/r_\mathrm{eff,min}$>2), and, therefore, have a lower limit of $r_\mathrm{eff}$ determined from the \ne\ and \Ha\ emission (see Section\,\ref{sec:lowerlimits}). {\em Centre:} The effect of varying the effective radius for the unresolved \HII\ regions within the sample. We show the difference caused by assuming the value of the lower limit ($r_\mathrm{eff}^\mathrm{lim}$) and measured value ($r_\mathrm{eff}$). The increase in size has no effect on the thermal pressure, hence causing a horizontal shift in the points (shown in blue). However, the $r_\mathrm{eff}^{-2}$ dependence in the $P_\mathrm{dir}$ calculation causes both a horizontal and vertical shift for the direct radiation pressure (shown in orange). Accounting for these lower limits will then always result in larger thermal pressures relative the direct radiation pressure. {\em Right:} The effect of varying the assumed conversion between \Ha\ luminosity (\LHa) and bolometric luminosity (\Lbol), which is used in the determination of the direct radiation pressure. Here we show the direct radiation pressure (blue points), and, for comparison, the thermal pressure (orange points) as a function of the effective radius. Throughout this work we have assumed a conversion of \Lbol\,$\sim$18\LHa, which accounts for the luminosity from only the ionising population. However, following \citet{kennicutt_2012}, we could also make the assumption that all the light from a fully sampled stellar population contributes to the radiation pressure; i.e. \Lbolimf\,$\sim$138\LHa. Given that \pdir$\propto$\Lbol, using \Lbolimf would causes a vertical shift of all the \pdir points on this plot.}
    \label{fig:limits}
\end{figure*}

==> figs/fig_presscatindv.tex <==
% \begin{figure*}
%     \centering
% 	\includegraphics[width=\textwidth]{./figs/scatter/rad_pallindv_pdeclass_compressed.pdf}
%     \caption{The various pressure components as a function of the effective radius for each galaxy in the sample. We show the internal pressure components of the direct radiation pressure (\pdir) and thermal pressure from the ionised gas (\ptherm) as orange and blue points, and the external confining pressure, or dynamical pressure (\pdess), as the green points.}
%     \label{fig:fig:scat_P_indv}
% \end{figure*}

% \begin{figure*}
%     \centering
% 	\includegraphics[width=\textwidth]{./figs/scatter/Rgal_pallindv_pdeclass_compressed.pdf}
%     \caption{The various pressure components as a function of the galactocentric radius for each galaxy in the sample. We show the internal pressure components of the direct radiation pressure (\pdir) and thermal pressure from the ionised gas (\ptherm) as orange and blue points, and the external confining pressure, or dynamical pressure (\pdess), as the green points.}
%     \label{fig:fig:scat_P_indv}
% \end{figure*}

==> referee_report.tex <==
We would like to thank the referee, Sebastian Sanchez, for taking the time to thoroughly read our manuscript, and to provide us with detailed comments and suggestions for improvement. We have taken these into account in the revised draft, which we believe has benefited from the referee's input. We hope that this revision now warrants publication in MNRAS.

Please find below a discussion of each of the referee's points. 

All changes made within the draft are highlighted in red.

We apologise that the previous version of the abstract was over the word limit. This has now been reduced to 247 words without loss of content. 

Major comments:

A) Authors gives a lot details to explain how the different internal
pressure components are derived. However, for the external pressure, P_de,
they give a set of references, but no actual formulae is provided.
I think it is important to explicitally quote the formulae adopted
and how the different parameters entering in that formulae are derived
from the data. In this regards I think they should follow Barrera-Ballesteros
et al. 2021, in which the different derivations and the actual equations
are provided (and the approximations).

For instance, reading 2nd paragraph, left column, of Page 16, it gives
the impression that the P_de is derived using a proxy combining the
stellar and gas surface densitites (e.g., like suggested by the results
in Barrera-Ballesteros et al. 2021b). It is that the case? This is
the kind of doubt that due to the lack of details in this derivation.

- We agree that this section was previously rather vague, and should have more explicitly clearly pointed to the work in Sun et al. (2020), from which the values we use are directly taken. We have now made this clearer, and provided a condensed version of the calculations presented within Sun et al., which we hope clarifies any confusion of how this parameter was determined (i.e. following the same method as Barrera-Ballesteros et al.). 

Furthermore, I do not see clearly stated (maybe it is and it escaped
to my supervision) why there are so many galaxies without an estimation
of P_de? 7/19 galaxies do not have it (Pg.19, left column). Why it is
so? Which measurements are required to derive this quantity. Why the
authors do not use another gauge/proxy of P_de based entirely on the
IFS data? How this bias in the number of galaxies may affect the results?

- Sun et al. provide the values of dynamical pressure for a subset of the galaxies studied in our work. The galaxies without these measurements either have no available HI observations or lack any significant CO (2-1) emission - such is the case e.g. IC 5332. This is mentioned within the caption of each figure showing the Pde measurement separated by galaxy (e.g. Fig 10), but was previously somewhat buried within the text of the observations section. We have now split this paragraph out such that it is more easily noted to the reader. 

- There are 7 galaxies without Pde measurements: NGC1365, NGC1433, NGC1512, NCG166, NGC1672, and NGC7496 have no available high-resolution HI observations, and IC5332 has a lack any significant CO emission in the PHANGS-ALMA data. It is not clear how this would bias our results, although it would be interesting to obtain these measurements in future. For example, it would be interesting to make our analysis in e.g. NGC1365, given that it has the highest SFR, stellar, and molecular mass within the sample. 

B) How the Diffuse Ionized Gas component is removed from the flux
estimations? I only see the DIG mention in Sec. 5.5 and in a footnote
(quoting a submitted and not accesible by Belfiore et al. 2021),
but there is no prescription on how the DIG contamination is considered
and removed. Could the authors elaborate a bit more on that?
DIG contamination is an issue in this kind of explorations. See
for instance the effort devoted to that in Espinosa-Ponce et al. 2020
(using lower spatial resolution data). I think it is important to
give more details in this regards. How it would affect the Halpha flux?
How it would affect the SII ratio? 

- Although we do not directly account for the contribution of the DIG in our determination of the HII region line fluxes, this was taken into account in our source identification routine using the HIIphot package - published soon in Santoro et al. (2021). Given the high sensitivity of the MUSE observations, we were able to recover much of the extended emission around the compact HII regions, which we minimised in the selection of the source identification parameters. That said, the contribution of the DIG to the HII regions studied in this work is expected to be low, given that (as you point out in one of your later comments), we have explicitly chosen to study the brightest regions due to our high flux selection thresholds (e.g. see Fig C1 for histogram of HII region luminosities). We do have active efforts to try to correct for this small contamination within the collaboration, however, doing so is not trivial, and often introduces large uncertainties. Lastly, the physical interpretation of removing the DIG in our analysis is not clear. As the leakage of ionised gas from the HII regions is thought to be one of the main contributors to the DIG, yet this gas could still contribute to the pressure terms we measure. 

- Nonetheless, we expect that the introduction of the DIG into our analysis could have a number of effects, and study of these on a case-by-case basis is far beyond the scope of this work. For example, within the central region where the DIG can be high, we could get HII regions that appear larger, confused, and/or diluted into the DIG. Indeed we recently showed within the MW CMZ (Barnes et al. 2020) that the HII regions within this environment can be systematically smaller than in the disc. This would in effect cause our pressures to be underestimated. 

- We have now added a discussion of the DIG to section 2.3, where the HII region samples are introduced. And leave a discussion of these potential DIG effects and how they could be addressed in future to the open questions in the discussion.  

Minor comments:

1) Effects of incompleteness in the derived conclusions.  From the list
of detected Hii regions, the authors have a relatively small subsample
of regions with r_eff and n_e measured (e.g., Fig 1 and Fig. 2, Table 1).
How this bias may affect the result? In some galaxies the fraction of
regions with those parameters measuered is just 1/10th of the total
original sample of Hii regions. They discuss on Sec 5.2, 3rd paragraph
on this bias. However, I think they need to explicitally quote it
in the conclusions/discussion and give it more weight.

- Indeed, in this work we do not offer to provide an unbiased or complete sample of HII regions within each galaxy, rather we are limited to the brightest and largest HII regions. This is due to the limitation of the observations in terms of resolution, and due to our stringent flux thresholds. We now explicitly mention this within the first paragraph of the conclusions and quote the number in each sub-sample. This is also now mentioned at the end of section 3.2, when the samples are first summarised. 

2) The authors select those regions that fullfil the following criteria:
"(ii) We require all of the strong lines used to compute line ratio
diagnostics (see below) to be detected with signal-to-noise greater
than three."
This indeed introduce a well known bias that has been discussed in previous
articles. For instance in Sanchez-Menguiano et al. 2018, using MUSE data,
it was used just a 1sigma detection limit and errors were propagated.
The reason for that is that, for instance, when selecting a 3sigma
cut in Hbeta you are actually selecting Ha regions with an S/N of ~10.
This selection may exclude regions that are well detected (i.e.,
detected with a significance in Ha larger than 3), but slightly affected
by dust. This bias acts in a similar way when selecting regions with
a signal in [OIII] larger than 3. For regions in the central areas
of galaxies or in the interarm, where [OIII] may be nearly one order
of magnitude weaker than Hbeta, and at the same time the dust attenuation
is large (see Fig. 2 of Sanchez et al. 2015), impossing a 3sigma cut in this
line may exclude regions that would be clearly detected in Hb and Ha,
and even in [SII].
In summary, I think this selection may introduce a bias that could affect
the results. Could the authors discuss on that? Are they sure that this
selection does not introduce any significant bias in their results?
I think a better approach would be to use the lower number of selections
on the line and line ratios and propagate the errors along this study.

- Again, we do not claim to offer a complete sample of the HII region within these galaxies, and are indeed heavily restricted by our need to measure the extinction corrected line fluxes accurately. This then limits us to the brightest regions, and, hence, we're likely missing large lower surface brightness regions that are likely older and less pressurised. However, in practice, our sensitivity constraints do not have a significant impact on our analysis. In order for us to calculate ne_max for an HII region, we need to be able to distinguish the [SII] line ratio for this region from the low density limiting value at the 3 sigma level. This requirement biases us towards brighter regions, since faint regions have too large an error in the [SII] ratio to reliably distinguish them from the low-density limit. 

- On investigating this further, we have found that **all** of the regions that are bright enough for us to be able to safely measure ne_max are also bright enough that all of the diagnostic lines (including [OIII] and Hbeta) are detected with S/N > 3, i.e. dropping the sensitivity cuts adds no new regions to our sample of regions with ne_max. The impact on the set of regions with calculated values of ne_min is also small. To calculate ne_min, we need to be able to measure the size of the HII region, i.e. it must have an angular radius greater than the FWHM of the MUSE PSF. At the distance of the PHANGS-MUSE galaxies, this corresponds to a physical size of 50-100 pc, and so we are only able to measure values of ne_min for relatively large HII regions. These tend to be bright, thanks to the well known HII region size-luminosity correlation, and in practice only 19 regions have a size large enough to measure while also having S/N < 3 in one of the diagnostic lines. Therefore, omitting the sensitivity selection increases the number of regions with calculated ne_min from 5669 to 5688, a ~0.3 per cent change. We can, therefore, be confident that our requirement of S/N > 3 for the diagnostic lines does not introduce any additional bias into our results.

3) Authors select the Hii regions based just on their location in the
BPT diagram. However, it is well known that other sources of ionization
may populate that region (see Sanchez 2020 and references in there).
The fact that you have selected clumpy (peaky) ionized regions using
HIIphot mitigates this effect, and the extremelly high S/N cut in Halpha
may also soften the problem. However, it is a good practice to select
as Hii regions only those regions within the selected area in the BPT
that fulfill other requirements, like having a large EW(Ha), and in particular,
for IFU data, a significant fraction of young stars (e.g., following
Espinosa-Ponce et al. 2020). Have the authors guaranteed that the
fraction of young stars at the location of the selected candidates
to Hii regions is large enough to produce the observed ionization?
I am particularly worried about other sources of ionization, like
shocks, that may affect the results somehow.

- Indeed, the source selection routine, which focuses on compact emission, and the high thresholds used in our work should mitigate contamination from other sources of ionisation. Nonetheless, there are currently ongoing efforts within the group to compare the young stellar populations and ionised gas distributions across the galaxy to confirm the HII regions. This, however, is a somewhat complex analysis beyond the scope of this work, and will be the focus of future publications. In fact, as noted within the future avenues (section 5.5), this is something that we are following up on using the available cluster catalogues from the higher resolution HST observations (Lee et al 2021). We have now also noted this within the introduction of the BPT diagnostics. 

4) I am a bit puzzled about the reported distributions of [SII] line
ratios in Fig. 4. The sampple of Hii regions seems to be dominated by
objects with a line ratio just at the edge at which the [SII] ratio is
sentitive to the electron density, peaking at line ratio of ~1.5,
corresponding to very low dense Hii regions.  My own experience is
that in general the distribution is flatter, from the samples I have
analyzed (e.g., Sanchez et al. 2012, Sanchez et al. 2015, Fig 2, or the
catalog by Espinosa-Ponce et al. 2020). For those samples the line
ratios suggest an average n_e ~ 300 cm^-3, corresponing to the
line ration of the sulfur doublet ~1. Could the authors offer
an explanation for this discrepancy? A possible reason could be
that they are exploring Hii regions in a sample of limited to late-type
galaxies (Sc/Sd), excluding inter-arm and central Hii regions in general.
Is that a possibility? A bias in the sample? I have not seen
in the article a clear description of the sample selection, that
it is refereed to Leroy et al. article. However, for the covered
cosmological distance the sample should be biased since they
selected objects inside the local cosmological fluctuation, no?
Could the authors discuss on that? It is an effect of the selection
of galaxies or a selection of Hii regions?

Another possible explanation is rather the oposite. I.e., an issue
with the reported results based on CALIFA and similar spectral resolution
data. It is possible that the lower resolution spectroscopic data are biasing
the published results towards lower values of the sufer doublet ratio?

In any case, I think the authors could discuss on this discrepancy offering
possible explanations.

- Indeed the galaxy sample is biased towards nearby, star-forming disc galaxies, which were chosen to allow us to study the sites of star formation at high linear resolution. The galaxy sample selection criteria are thoroughly outlined in both the PHANGS-ALMA (Leroy et al. 2021) and PHANGS-MUSE survey papers (Emsellem et al. 2021). 

- In general, we are not excluding the galaxy centres, as these are typically some of the brightest regions, and hence meet our selection criteria (e.g. see Figure 1). We see that these central regions typically have HII regions with the highest electron densities, as highlighted by the increase in the thermal pressure at low Rgal/Reff (e.g. Fig 12). That said, the centres are particularly confused regions, due to the number of HII regions within a small volume and the increase DIG level. Hence, as previously noted, it could be that the [SII] doublet fluxes are diluted within this region, and the ne measurements are underestimated. That said, it is not possible to study here this due to the resolution limitations of the MUSE observations, and hence we have noted this is as an avenue for future observations.

- With regards to the literature comparison, our measurements of the electron density from the SII doublet are in the range 30 - 300 cm^-3 (see ne_max in Fig. 6). We do not see these values as unreasonable given the large sizes of the HII regions (~>50pc), and, for the most part, these electron densities provide a Ptherm that is ~Pde. A significant increase in the electron densities to >300 cm^-3 could present a problem, as this would cause the HII regions to become highly overpressured, which one would not expect to be the case in large, evolved HII regions. We also note that the values of the [SII] ratio that we find in our study seem to be in good agreement with those derived in other IFU studies of HII regions in nearby spiral galaxies (see e.g. the results shown in Rousseau-Nepton et al 2018 for NGC 628, or those reported by McLeod et al. 2020 for NGC 300).

- The comparison with the lower resolution studies you mention is, however, an interesting avenue to follow in future, and we have noted this within the text (section 3.2). 

5) How the electron densities derived from the SII ratio compares with
those derived based on Q for thos regions with both measurements in
common? I understand their are minimum and maximum electron densities,
but I think it would be really illustrate to show a comparison. The
same for the effective radius derived using the using the electron
density or directly measured (when the resolution allows it). Could
the authors provide with this comparison?

- We now provide a comparison between the minimum (derived from the Ha emission and the measured size) and maximum (derived from the SII ratio) electron densities in Figure A1. Here we see that these two measurements have a ratio of around a factor of ten, highlighting that the volume filling factor of the unresolved HII regions could be around ~1per cent. Constraining the sizes (i.e. the volume filling factor) for a sample of these HII regions using higher angular resolution HST observations is something that we're now actively following up (mentioned in section 5.5). 

6) When the authors derive the Thermal gas pressure the assume
a value of Te=8000 when they cannot derive the Te from the auroral
lines. However, it would be equally right to use the minimum and
maximum values in the measured Te distribution (6000-16000 K), an use
this range to derive the minimum and maximum pressure, no?
I mean, using Te=6000 and ne_min would produce a lower P_therm,min
than the currently derived, no? In the other hand, using Te=16000K and
ne_max would produce a higher P_therm,max? I do not think this would
change the result, but I would produce a more consistent value following
the argumentation by the authors.

- We agree that including these additional limits into the measurement of the Ptherm would be a good idea, and something that we have looked into. However, we decided against this as this could over-complicate the analysis, providing an additional set of limits (along with the size and ne) that would not affect our analysis. Ultimately, the dominant source of uncertainty is from the limits imposed from the sizes and electron density measurement (as these are not linear), whereas a change in the electron temperature of around a factor of 2 (6000-16000 K) would only produce a variation in the thermal pressure of the same factor. For simplicity, we have then chosen to keep a constant Te where no measurement is available. 

7) Sec. 4.2, 1st and 2nd paragraph. I think in this regards the authors
should acknowledge the recent results on the topic by Barrera-Ballesteros
et al. 2021 (quoted below). I think it is important to compare with the
values reported using other datasets and approaches to derive P_de to
compare with. Are the values of the same order? Are they different?
Why?

- We have taken the values of Pde directly from Sun et al, who Barrera-Ballesteros et al. 2021 already make a comparison with (e.g. their Figure 9). We have added a citation to this work, but as the dynamic pressure estimates have already been analysed in detail, and these are not the focus of this work, we have not included an in-depth comparison here.

8) Fig. 12. Normalizing the radial gradients to R25 is a procedure
that was long adopted. However, more recent explorations adopt a normalization
that depends less on the shape of the radial profile and the distance, like
the effective radius. Have the authors consider that possibility?

- We have updated all plots to normalise to the Reff from PHANGS-ALMA survey paper (Leroy et al. 2021). The values of the Reff are also now provided in Table 1.

9) Fig. 12. Note that the radial gradient of P_de is expected as the
combination of the stellar and gas surface densities are a tracer of this
quantity. It is expressed somehow when discussing this Fig. in Pg. 16.
If the derivation of P_de is independent of those parameters (see my
major comment in this regards), they authors could indeed compare both
quantities and explore if they have the expected correspondence suggested
in the literature. This will give support to their derivation of P_de.

- Indeed the Pde increases towards the centre of the galaxies, where both the stellar and gas surface densities are higher. We hope this is now clear from the addition of the derivation of Pde in section 2.3 (relating to you second major comment).

10) When quoting the effect of feedback in the molecular gas cycle
and the star-formation process I think it is relevant to quote the two
articles indicated before by Barrera-Ballesteros et al. 2021,2021b.
These results are also relevant in the discussion included in Sec. 5.5,
pg. 23, left column, when addressing the pressure balance at kpc-scales,
and in the Summary (Sec 6, 2nd paragraph).

- We apologise for missing these references, which are now included in the initial introduction of the dynamical pressure, and the discussion and conclusions section where you suggest.

Final note on the style:

I have a final note, but is a rather personal appreciation and it
should be the editor who should give a word on that: I think the style
adopted for the figures is more appropiate for a poster than for an
article. Sometimes I think there is a bit of over-doing with the
colors, style of the legends and so on. On the contrary sometimes
there are some style errors. For instance, in the left-side label of
Fig. 13 is missplaced, producing an extra space in the top of the
figure. I have the impression that too much detail is given to the
inner part of that figure but less to the outer part.

I have to admit that this is personal perspective and if the editor
is ok with this style I would say nothing else in this regards.

- We appreciate your opinions on the styling of the figures, which we purposefully produced to be over-explicit to help the reader understand what was plotted at a glance. We have discussed this issue internally and decided that, if the editor is happy with the current styling, we will keep them in the current form.  

- In addition, we appreciate your diligence in checking the figures and highlighting the issue with Figure 13, which has now been updated.

Relevant references that could be useful:

Barrera-Ballesteros et al. 2021
https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.3643B/abstract

Barrera-Ballesteros et al. 2021b
https://ui.adsabs.harvard.edu/abs/2021ApJ...909..131B/abstract

Espinosa-Ponce et al. 2020
https://ui.adsabs.harvard.edu/abs/2020MNRAS.494.1622E/abstract

Sánchez et al. 2012
https://ui.adsabs.harvard.edu/abs/2012A%26A...546A...2S/abstract

Sánchez et al. 2015
https://ui.adsabs.harvard.edu/abs/2015A%26A...574A..47S/abstract

Sanchez-Menguiano et al. 2018
https://ui.adsabs.harvard.edu/abs/2018A%26A...609A.119S/abstract

Sánchez et al. 2021
https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.1615S/abstract

Sánchez 2020
https://ui.adsabs.harvard.edu/abs/2020ARA%26A..58...99S/abstract

We have included all of the above references where relevant. 



==> tabs/tab_obsprops.tex <==
\begin{table*}
\centering
    \caption{Observational properties of \HII\ regions sample for all galaxies. This sample includes the $\sim$5000 \HII\ regions that meet the selection criteria outlined in Section\,\ref{sec:selection_bias} (i.e. those that meet the limiting conditions a, b, and c). This table is provided in full machine readable format in the online supplementary material. The properties of the full nebula catalogue for the galaxy sample studied here will be provided by Belfiore et al. (in prep).}
    \label{tab:obsprops}
    
\begin{tabular}{ccccccccc}
\hline \hline
Galaxy & ID & RA & DEC & $r_\mathrm{eff}$ & E(B-V) & $F_\mathrm{H\alpha}$ & $F_\mathrm{[SII]\lambda6716}$ & $F_\mathrm{[SII]\lambda6731}$ \\
 &  & $\mathrm{{}^{\circ}}$ & $\mathrm{{}^{\circ}}$ & $\mathrm{{}^{\prime\prime}}$ & $\mathrm{mag}$ & $\mathrm{erg\,s^{-1}\,cm^{-2}}$ & $\mathrm{erg\,s^{-1}\,cm^{-2}}$ & $\mathrm{erg\,s^{-1}\,cm^{-2}}$ \\
 \hline
IC5332 & 2 & 353.595 & -36.084 & 1.287 & 0.153 & 642191.6 & 55638.6 & 38992.4 \\
IC5332 & 8 & 353.624 & -36.078 & 0.814 & 0.115 & 143075.3 & 22310.4 & 15389.7 \\
IC5332 & 11 & 353.617 & -36.101 & 0.910 & 0.113 & 71449.0 & 14075.5 & 9447.7 \\
IC5332 & 16 & 353.623 & -36.089 & 0.837 & 0.118 & 191819.8 & 24487.5 & 16872.7 \\
IC5332 & 17 & 353.614 & -36.103 & 1.022 & 0.137 & 313153.7 & 45164.7 & 30686.9 \\
IC5332 & 18 & 353.598 & -36.079 & 0.881 & 0.089 & 69624.3 & 23073.8 & 16114.1 \\
\dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots \\

\hline
\end{tabular}
\end{table*}

==> tabs/tab_physprops.tex <==
\begin{table*}
\centering
    \caption{Physical properties of the \HII\ region sample. We provide both the value or, where applicable, the upper or lower limit estimate of the derived physical quantity. This table is provided in full machine readable format in the online supplementary material.}
    \label{tab:phyprops}

\begin{tabular}{cccccccccccccc}
\hline \hline
Galaxy & ID & $R_\mathrm{gal}$ & $r_\mathrm{eff}$ & $r_\mathrm{eff}^\mathrm{lim}$ & $n_\mathrm{e}$ & $n_\mathrm{e}^\mathrm{lim}$ & $P_\mathrm{dir}$ & $P_\mathrm{dir}^\mathrm{lim}$ & $P_\mathrm{wind}$ & $P_\mathrm{wind}^\mathrm{lim}$ & $P_\mathrm{therm}$ & $P_\mathrm{therm}^\mathrm{lim}$ & $P_\mathrm{de}$ \\
  & & & & & & & log() &  log() &  log() &  log() &  log() &  log() &  log() \\
 &  & $\mathrm{kpc}$ & $\mathrm{pc}$ & $\mathrm{pc}$ & $\mathrm{cm^{-3}}$ & $\mathrm{cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ & $\mathrm{K\,cm^{-3}}$ \\
 \hline
IC5332 & 2 & 3.66 & 51.0 & - & - & 2.7 & 3.33 & - & 4.34 & - & - & 4.62 & - \\
IC5332 & 8 & 3.69 & 32.3 & - & - & 2.6 & 3.07 & - & 4.08 & - & - & 4.59 & - \\
IC5332 & 11 & 0.34 & 36.1 & - & - & 1.5 & 2.67 & - & 3.69 & - & - & 4.37 & - \\
IC5332 & 16 & 2.09 & 33.2 & - & - & 2.8 & 3.17 & - & 4.19 & - & - & 4.63 & - \\
IC5332 & 17 & 0.31 & 40.5 & - & - & 2.7 & 3.21 & - & 4.23 & - & - & 4.61 & - \\
IC5332 & 18 & 4.09 & 35.0 & - & - & 1.6 & 2.69 & - & 3.70 & - & - & 4.38 & - \\

\dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots \\


\hline
\end{tabular}
\end{table*}

==> text/intro_old.tex <==
\section{Introduction}

\input{./figs/fig_map.tex}

High-mass stars (>8\,\sol) inject a large amount of energy and momentum---stellar feedback---into the interstellar medium (ISM) during their relatively short lifetimes. The feedback from these stars can influence the ISM both locally (<1\,pc) and on kpc scales, via a variety of processes (e.g. \citealp{krumholz_2014}). It appears that the most important of these feedback mechanisms for the overall momentum budget of the ISM occurs at the end of the stars lifetime, when they explode as supernovae (SNe; \citealp{mckee_1977,maclow_2004,klessen_2016}). The momentum injection from SNe is suggested to be one of the main mechanisms driving the turbulence in molecular clouds, which limits the rate at which stars can form from the ISM (e.g.\ \citealp{hennebelle_2011, federrath_2012, federrath_2013a, Padoan2017, Dekel2019}). However, simulations (e.g.\ \citealp{dale_2012, dale_2013, Gatto2017, Rahner2017, Rahner2019, Kannan2020}) suggest that in fact feedback in the early evolutionary stages (pre-SN) of stars  plays a critical role in regulating the star formation process. Indeed, \ch{recent observations measured rapid (1 to 5\,Myr)} destruction of molecular clouds, implying that stellar winds, photoionized gas, and (direct and indirect) radiation pressure from young stars may play a dominant role in halting star formation, and limiting the overall efficiency at which molecular clouds can be converted to stellar clusters (e.g.\ \citealp{kruijssen19a,chevance20b,chevance20,Kim2020}). Understanding which mechanism dominates early-stage stellar feedback is therefore of crucial importance for a complete picture of the self-regulatory star formation cycle.


%Simulations show that this this SNe is relatively insensitive to the host environment (e.g.\ \citealp{Kim2015,Kim2017,Walch2015,Martizzi2015,Iffrig2015}.

The qualitative effect of pre-SN processes has been well studied for several decades, but a quantitative analysis focusing on the physical properties of a large sample of young star-forming regions has yet to be undertaken. Recent efforts have focused on measuring and comparing the internal pressure components from different feedback mechanisms within \HII\ regions; i.e.\ regions containing a high ionisation hydrogen fraction, indicating the presence of high-mass star(s). While informative, these studies have focused on relatively small samples of \HII\ regions across the Milky Way (e.g.\ \citealp{barnes20b, olivier2020}), the Small and Large Magellanic Clouds \citep{lopez_2011, lopez_2014, Pellegrini2012, chevance16, mcleod_2019}, and in the nearby galaxy NGC300 \citep{mcleod_20}. Further work is needed to increase this sample and systematically investigate how pre-processing varies with galactic environments and between galaxies.

\ch{In order to investigate the relation between pre-SN feedback and the galactic environment, this paper aims to assess the various} internal and external pressure components within a sample of several thousand \HII\ regions identified across 19 nearby spiral galaxies. Table\,\ref{tab:galprops} provides an overview of the global properties of this sample. This work exploits optical integral field spectroscopy from the Multi Unit Spectroscopic Explorer (MUSE; \citealp{bacon10}) instrument mounted on the Very Large Telescope (VLT). The spatial sampling and large field of view of MUSE allow us to analyse the properties of the ionized gas at high resolution ($\sim$\,50--100\,pc) in even in systems as far as 19\,Mpc. \ch{These observations were taken as part of the Physics at High Angular resolution in Nearby GalaxieS (PHANGS)\footnote{\url{https://sites.google.com/view/phangs/home}} collaboration, which combines large programmes on ALMA \citep{Leroy2021}, MUSE (Emsellem et al. submitted), and HST \citep{Lee2021}, as well as a variety of ancillary multi-wavelength data, to assess the star formation, molecular gas, and stellar cluster properties across a large sample of nearby galaxies.} The synergy between these observations is fundamental to calculating and assessing how the internal and external pressure components of \HII\ regions vary as a function of the galactic environment.

This paper is organised as follows. In Section\,\ref{sec:sampleselection}, we introduce the sample 19 nearby galaxies and MUSE observations that are used to identify and study their \HII\ region populations. In Section\,\ref{sec:physprops}, we outline assumptions for the unresolved density distribution within each of the identified \HII\ regions, and use these to estimate their physical properties. In Section\,\ref{sec:prescalc}, we place limits for the internal pressures within each \HII\ region. We compare how the pressure components vary across the galaxies, how the total internal pressure compares to the external pressure, and how these results compare to samples within the literature in Section\,\ref{sec:prescomp}. Finally, the main results of this paper are summarised in Section\,\ref{sec:summary}.


%AL : I'll send a high level note, and you can totally ignore, but this section chooses a weird tone. It's very oriented towards SNe or not. HII regions are a thing, they grow and get big, massively affecting the surrounding ISM. That's just a thing. I think a sketch of the growth of HII regions from compact to big and evolved, with a note on the physical processes involved - tell us about thermal pressure, winds, radiation pressure. The fact that it's NOT SN occupies a huge amount of the space here? That's really good to mention but the focus seems off. I would spend this spot to at least introduce the readers to the key physical processes you DO analyze

==> text/summary_old.tex <==
\section{Summary}\label{sec:summary}

In this paper, we compare the internal and external pressures acting on a sample of $\sim$\,6000 \HII\ regions across 19 nearby spiral galaxies. The \HII\ region sample is identified using Multi Unit Spectroscopic Explorer (MUSE) data taken as part of the Physics at High Angular resolution in Nearby GalaxieS survey (PHANGS-MUSE; Emsellem et al. A\&A subm.). We place upper/lower limits on the internal pressure components of the thermal pressure from the warm ionised gas (\ptherm; Section\,\ref{sec:therm_prescalc}), direct radiation pressure (\pdir; Section\,\ref{sec:dir_prescalc}), and mechanical wind pressure (\pwind; Section\,\ref{sec:wind_prescalc}), which we compare to the confining external pressure of their host environment, or their dynamical pressure (\pde; Section\,\ref{sec:ext_prescalc}). With the MUSE observations, we cannot constrain the unresolved density distribution within the ionised gas, and hence we place upper and lower limits on each of the internal pressure components. The lower limit (\pmin) corresponds to the assumption of a smooth density profile, where the measured radius (\reff) is assumed to be representative of the \HII\ volume over which the pressure is acting (Section\,\ref{subsubsec:reff}). The upper limit (\pmax) corresponds to the assumption of a more clumpy density profile, where the minimum radius (\rmin) is derived from the electron density measurement (Section\,\ref{sec:lowerlimits}). The main conclusions of this work are summarised below. 

We assess the relative differences of the \pmax\ or \pmin\ measurements for each pressure term. We see that the maximum internal pressures are all relatively similar, with mean values of around $\pmax/k_\mathrm{B} \sim 10^{6}$\,\Kcmcb. On the other hand, the minimum values appear relatively different, with the direct radiation and wind pressures having values around $\pmin/k_\mathrm{B} \sim 10^{4}$\,\Kcmcb\ and the thermal pressures being around a factor of~4 higher ($P_\mathrm{therm,min}/k_\mathrm{B} \sim 10^{4.6}$\,\Kcmcb). This shows then that at best the pressure terms are comparable if they have a compact density distribution (i.e. at \pmax). However, it is likely that the vast majority of \HII\ regions are likely to have at least some extended structure (i.e. tending to $\pmin$) that would then cause \ptherm\ to become dominant. 

Comparison to a sample of \HII\ region pressure measurements available within the literature shows that on the scales of several tens to a couple of hundred parsecs \ptherm\ is expected to be the highest internal pressure (e.g. \citealp{lopez_2011, lopez_2014, mcleod_2019, mcleod_20}). In addition, we compare to \HII\ regions within the Milky Way and more nearby galaxies such as the LMC and SMC; combined with the presented measurements of this work, this combined sample covers a total of six orders of magnitude in spatial scale ($0.001$ to $300$\,pc). Indeed, above scales of around~$0.1$ to~$1$\,pc the thermal pressure is marginally dominant, yet below $0.1$\,pc the direct radiation pressure is dominant \citep{lopez_2014, mcleod_2019, barnes20b, olivier2020}. We note that due to inconsistencies within the literature, this comparison does not include the indirect (trapped) radiation pressure from heated dust or the contribution of winds.

We compare our total internal pressures within each \HII\ region to the external external pressure ($\ptot = \ptherm + \pdir + \pwind$) of their host environment taken from \citet{sun20}. We see that for the $P_\mathrm{tot,min}$ limits (see Figure\,\ref{fig:scat_PtotPDE}) just under half of the \HII\ regions ($1927$ in total) are over-pressured relative to their environment (i.e. $P_\mathrm{tot,min} > \pde$). These \HII\ regions would still be expanding despite their large measured sizes of several tens to a few $100$\,pc (\reff), and would, therefore, represent interesting targets to study the effect of large-scale expansion in the (ionised, atomic and molecular) gas spatial and kinematic distributions. The remaining $2206$ \HII\ regions appear to be under-pressured relative to their environment, highlighting that these have most likely stopped expanding.

We see that for the $P_\mathrm{tot,max}$ limits, the majority of \HII\ regions are now over-pressured. This is expected as $P_\mathrm{tot,max}$ is estimated assuming an \HII\ region size scale typically of the order a few to a few tens of parsecs. In this case, \HII\ regions would be still relatively young and expanding. Interestingly, however, there is a small number of compact \HII\ regions~(15) that are under-pressured relative to their environment. Plotting the ratio of the internal pressure over the external pressure, $\log(\ptot/\pde)$, as a function of galactocentric radius (see Figure\,\ref{fig:scat_PtotPDEreff}), we see that the majority of these compact under-pressured \HII\ regions reside within galaxy centres. This then highlights that centres are interesting high-pressured regions in which to assess the effects of stellar feedback \citep[see e.g.][]{barnes20b}. To assess more generally, we investigate if the increase in gas density has a significant effect on the over- (under-) pressured nature of an \HII\ region (see Figure\,\ref{fig:scat_PtotSigma}). We see that regions of galaxies (or environments in general) with higher gas surface densities have fewer over-pressured \HII\ regions (and more under-pressured \HII\ regions). The simple interpretation of this is that a more dense environment may inhibit rapid expansion, and thus limit the effect of stellar feedback. This is of particular importance not only for current-day star formation, but also have implications for cosmic timescales, given that ISM pressures and densities observed at the peak of the cosmic star formation history are several orders of magnitude higher than those observed in disc galaxies today \citep[e.g.][]{genzel11,swinbank11,swinbank12,tacconi13}. 

In all, this work demonstrates that the balance of internal and external pressures for \HII\ regions varies strongly both between galaxies and within galaxies (i.e. with environment). We note that within this work, we had to make several simplistic assumptions about the potentially unresolved sub-structure of \HII\ regions within our sample. This then presents a simple requirement for higher-spatial resolution data sets in future, either from higher-angular resolution observations (e.g.\ from the {\em Hubble Space Telescope}) or integral field spectroscopy observations of more nearby targets (e.g. SIGNALS and the \mbox{SDSS-V} Local Volume Mapper survey; \citealp{Kollmeier2017}).

% \begin{itemize}
%     \item[(i)] Comparing the various internal pressure components, we find that \ptherm, \pdir\ and \pwind\ have mean values of $\mathrm{log}(P/k_\mathrm{B})\,\sim\,5.9$\,\Kcmcb, 5.4\,\Kcmcb\ and 3.9\,\Kcmcb, respectively. Therefore, on the scales of 20--400\,pc probed by our \HII\ region sample, we find that the thermal pressure is the dominating internal pressure component by one to two orders of magnitude. We find that \ptherm>\pwind>\pdir\ is systematic across all individual galaxies within our sample.    
%     \item[(ii)] We find a mean $\mathrm{log}(P_\mathrm{DE}/k_\mathrm{B})\,\sim\,5.2$\,\Kcmcb, and typically \ptherm>\pde>\pwind>\pdir\ across the galaxy sample. Comparing the total internal pressure (\ptot=\ptherm+\pdir+\pwind) to the external pressure, we find that \HII\ regions are typically over-pressured by around a factor four ($P_\mathrm{tot}/P_\mathrm{de}\,\sim\,4$). However, this varies significantly across the sample. We find that \HII\ regions within lower external pressure environments are typically over-pressured ($P_\mathrm{tot}/P_\mathrm{de}\,\sim\,1000$), whilst those within higher-pressure external environment are under-pressured ($P_\mathrm{tot}/P_\mathrm{de}\,\sim\,0.1$). As \ptot\ is relatively constant for a large variation in \pde, this suggests that the expansion and dynamics of \HII\ regions from tens to hundreds of parsec scales are determined not by the internal properties of the \HII\ region, but the environment in which it expands into. Interestingly, these high ambient pressures are typically located towards the centres of the galaxies, which could highlight these environments as interesting regions for future studies of feedback (also see \citealp{barnes20b}).
%     \item[(iii)] We compare our sample of $\sim$\,5000 \HII\ regions to the $\sim$\,300 currently available with similar measurements within the literature \citep{lopez_2014, mcleod_2019, barnes20b, olivier2020}. This literature sample includes \HII\ regions across the Milky Way and nearby galaxies such as the LMC and SMC, and covers six orders of magnitude in spatial scale. Comparing \pdir\ and \ptherm, we see that the relative contribution of the pressure components varies as a function of \HII\ region size. Above scales of around 1\,pc the thermal pressure is dominant, yet below 1\,pc the direct radiation pressure is dominant. Due to inconsistencies within the literature, this comparison does not include the indirect radiation pressure from heated dust, or the contribution of winds. 
% \end{itemize}
